Pulse Shape Discrimination and Exploration of Scintillation Signals Using Convolutional Neural Networks

We demonstrate the use of a convolutional neural network to perform neutron-gamma pulse shape discrimination, where the only inputs to the network are the raw digitised SiPM signals from a dual scintillator detector element made of 6LiF:ZnS(Ag) scintillator and PVT plastic. A realistic labelled dataset was created to train the network by exposing the detector to an AmBe source, and a data-driven method utilsing a separate PMT was used to assign labels to the recorded signals. This approach is compared to the charge integration and continuous wavelet transform methods and is found to provide superior levels of discrimination, achieving an AUC of 0.995 +/- 0.003. We find that the neural network is capable of extracting interpretable features directly from the raw data. In addition, by visualising the high-dimensional representations of the network with the t-SNE algorithm, we discover that not only is this method robust to minor mislabeling of the training dataset but that it is possible to identify an underlying substructure within the signals that goes beyond the original labelling. This technique could be utilised to explore and cluster complex, raw detector data in a novel way that may reveal more insights than standard analysis methods.

==> Sections/section3_2.tex <==
\subsection{Unsupervised learning}
\label{Unsup}

As structured series of elements, the waveforms could be considered high dimensional vectors that would be expected to form two major clusters representing the two major signal types. Accurate clustering is a non-trivial problem that is intuitively worsened by the presence of redundant, non-distinguishing information within the signal waveforms. As compressed representations of the waveforms encoding the least redundant information, applying clustering techniques to latent vectors was considered a method to circumvent these problems.
\\
\\
To demonstrate the operation of a latent vector as a compressed representation and the importance of its size, twenty networks were trained for each viable pooling factor between 2 and 12. To compare and contrast the results, a metric as required for the quality of the waveform reconstruction at the system output which, to be most informative, would not be incorporated into the loss function itself. For this purpose, the relative change in vector magnitude and the normalised cross correlation between the autoencoder input and output were considered. In practice, the change in vector magnitude did not vary significantly between autoencoder architectures and was neglected. As the pooling factor was increased, the distributions of normalised cross correlations worsened consistently in line with the increased compression of any lossy compression method. Due to the higher volume of information contained within a neutron signal, these waveforms were more significantly affected by the change in pooling factor. \textbf{(Require figures here)}
\\
\\
To demonstrate the viability of labelling signal waveforms by clustering latent vectors, a greedy clustering algorithm was applied to the resulting latent vectors of the pooling investigation described above that clustered based on each vectors angular position. This algorithm was unstable when applied to the signal waveforms directly. The resulting ROC curves were compared to the AUC of the traditional methods described in section 2. \textbf{(Could use table here)}. Using a pooling factor of 2, 55\% of networks resulted in a superior AUC to traditional methods. This consistently increased to a value of 85\% using a pooling factor of 12. Of these superior networks using a pooling factor of 12, the mean average AUC was 0.982 $\pm$ 0.006. 



